The Impacts of Dimensionality, Diffusion, and Directedness on Intrinsic Cross-Model Simulation in Tile-Based Self-Assembly

Algorithmic self-assembly occurs when disorganized components autonomously combine to form structures and, by their design and the dynamics of the system, are forced to follow the execution of algorithms. Motivated by applications in DNA-nanotechnology, investigations in algorithmic tile-based self-assembly have blossomed into a mature theory with research leveraging tools from computability theory, complexity theory, information theory, and graph theory to develop a wide range of models and show that many are computationally universal, while also exposing powers and limitations of each. Beyond computational universality, the abstract Tile Assembly Model (aTAM) was shown to be intrinsically universal (IU), a strong notion of completeness where a single tile set is capable of simulating all systems within the model; however, this result required non-deterministic tile attachments. This was later confirmed necessary when it was shown that the class of directed aTAM systems is not IU. Building on these results to further investigate the impacts of other dynamics, Hader et al. examined several tile-assembly models which varied across (1) the numbers of dimensions used, (2) restrictions based on diffusion of tiles through space, and (3) whether each system is directed, and showed which models are IU. Such results have shed much light on the roles of various aspects of the dynamics of tile-assembly and their effects on the intrinsic universality of each model. Here we provide direct comparisons of the various models by considering intrinsic simulations between models. We show that in some cases one model is more powerful than another, and in others, pairs of models have mutually exclusive capabilities. This comparison helps to expose the impacts of these three important aspects and further helps define a hierarchy of tile-assembly models.

==> DP3DaTAM-not-IU.tex <==
\section{The Directed Spatial aTAM is not IU}

In this section, we prove that there is no tile set which is intrinsically universal for the set of directed systems within the Spatial aTAM.

\begin{theorem}\label{thm:DS3DaTAM-not-IU}
The class of directed systems in the Spatial aTAM is not IU.
\end{theorem}

\begin{proof}
Our proof will be by contradiction, so assume that the class of directed systems in the Spatial aTAM is IU and that $U$ is a universal tile set for this class. We will present a system $\calT$ in that class such that $U$ cannot correctly simulate $\calT$.



% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{3.0in}
%         \centering
%         \includegraphics[width=1.8in]{images/ring1.png}
%         \caption{An example of a box lid which has a ring at radius 6. Note how the orange tile of a lid protrudes one extra location (as does its neighbor, which attached first and allowed it to bind and then possibly seal a box region).}
%         \label{fig:ring1}
%     \end{subfigure}
%     \hspace{0.2in}
%     \begin{subfigure}[b]{2.0in}
%         \includegraphics[width=1.8in]{images/ring2.png}
%         \caption{An example of a box bottom which has a ring at radius 4. Note how the orange tile of a bottom does not protrude like that of a lid.}
%         \label{fig:ring2}
%     \end{subfigure}
%     \caption{An example box lid and bottom of total radius 7 each, which have mismatching rings (and only one each) so if they were the two halves of a box, the box would not be sealed and the POC tile could be placed.}
% \end{figure}

First, we describe the system $\calT=(T, \sigma, 2)$. As an overview, $\calT$ is composed of an infinite grid of \emph{maze boxes}. Each maze box will be made up of two \emph{half mazes}, a \emph{top maze} and a \emph{bottom maze}. Each half maze is a square surface made up of \emph{panels} which are made up of tiles in a $5\times 5$ square with some tiles forming walls or cooperative binding points above or below the square for bottom or top half mazes respectively. There are 32 different panels and a half maze is simply a square arrangement of these panels. Note that a half maze is open on one side and so is not sufficient to constrain a subspace. When a top maze is grown above a bottom maze, they form a maze box which, depending on the specific half mazes, may constrain several subspaces and may contain several points of cooperation (\emph{POCs}).

\begin{figure}
    \centering
    \includegraphics[width=3.5in]{images/box-pixels.png}
    \caption{The set of all possible options for a pixel is the set of the three options on the left (for the $5\times5$ surface) crossed with the $15$ options on the right (for the presence or lack of each wall).}
    \label{fig:box-pixels}
\end{figure}


% The top half of each box is called a \emph{lid}, and the bottom half is called a \emph{bottom}. Each lid and bottom is grown independently, and at different offsets, so that lids and bottoms do not always align. Each consists of a flat surface as well as a series of concentric square \emph{rings} centered around the center point of the lid/bottom. Each ring of the lid extends one tile in the direction between the lid and bottom, and each ring of the lid extends two tiles in the direction between the bottom and the lid. The center position of each lid/bottom is a special ``orange'' tile which is placed one tile in the direction between them. If a lid and a bottom are aligned so that their centers, and thus their orange tiles, are directly across from each other, and both have at least one ring whose radius is equal, those rings will be touching for their entire length and will cause the box to be \emph{sealed}, i.e. once the orange tile, which is the last to be placed for each of a lid and bottom, has attached, the center of the box outward to a pair of rings with matching radii is a constrained subspace. However, if no pair of rings, one each from the lid and bottom, have matching radii, then there will be a minimum of a one-tile-wide path from completely outside the box all the way to the location between the orange tiles of the lid and bottom. Between them will be a one-tile-wide gap and they will be able to cooperate, via exposed strength-$1$ glues, to place a tile between them. That cooperatively placed tile will have an exposed $\tau$-strength glue which will allow a tile to attach to a side orthogonal to the sides attached by the orange tiles.

We now discuss how an infinite grid of maze boxes self-assemble in a way which ensures that $\calT$ is directed, but also with some additional aspects that ensure that a simulator must fail to correctly simulate all systems similar to $\calT$.

$\calT$ begins from a single seed tile at $(0,0,0)$, and from that tile an infinite log-width counter, starting at the value $8$, called the $\backbone$ grows in the $+x$ direction. The $\backbone$ increments every $\backinc$ tiles. At each $\backinc$th tile, the $\backbone$ grows a row of tiles encoding its current value, $n$, in the $-y$ direction that will become a $\bottomrib$ and a single tile in the $+y$ direction that will become a $\toprib$. Adjacent to the row of tiles growing into a $\bottomrib$, the $\backbone$ also grows a row of tiles encoding $n$ that will become the $\metarib$. Each $\bottomrib$ is a pair of fixed-width, cyclic counters. The first counter has a period of the value $n$ from the $\backbone$ and it counts infinitely often from $0$ to $n-1$. Each time, the first counter reaches $0$, the value of the second counter is incremented and rotated upward to be used as a seed value for growing a maze bottom.\todo{It sounds like the second counter increases infinitely, meaning that it can't be a fixed-width counter.} Each $\toprib$ contains a pair of log-width binary counters, one nested within the other. They both start at the value $8$ (i.e. $2^3$), and the value $i$ of the inner counter remains constant while the value of the outer counter, $j$ increments one value at a time until reaching the next power of $2$, $2^4$, at which point value of $i$ is incremented. The value of $i$ then remains constant until $j$ reaches the next power of $2$, and then $i = i + 1$. This process continues infinitely. Each time the value $j$ is incremented, its value is rotated and used as the input for a zig-zag Turing machine which computes the value to be used to seed the growth of a maze top.


Each $\metarib$ contains both the fixed-width, cyclic counters of the corresponding $\bottomrib$ and the pair of log-width binary counters of the $\toprib$. It uses these counters, along with its own zig-zag Turning machine to determine...
\begin{enumerate}
    

    % \item  [TODO: add more details about spacing and growth of box bottoms]
    
    % \item  [TODO: add details about spacing for boxes and describe the growth of box lids]. If the growth of a $\toprib$ was initiated from the $\backbone$ at value $n$, we refer to the box lid which grows when the inner counter is at value $i$ as $\texttt{box}(n,i)$.
    
    % \item  For each ...
    
    % \item TODO: describe the order of grow of a box lid/bottom, with the center, orange tile attaching last. A high-level depiction of the growth process can be seen in Figure~\ref{fig:ring-growth}.

    \item In the cases when the center of a box lid aligns with the center of a box bottom, we call the location inside the box and between the two orange tiles a \emph{point of cooperation} (POC), since the orange tiles can potentially cooperate to place a tile between themselves, assuming the POC is not located within a constrained subspace, a.k.a. a \emph{sealed} box (which is one where at least one wall of the box lib aligns with a wall of the box bottom, thus sealing the space inside of those walls). Note that the boxes are designed so that, iff the bit strings used to grow the top and bottom are equal, the box is not sealed and there is a diffusion path that allows a tile to attach in the POC. Otherwise, the box is sealed, and no tile can attach in the POC. We call the tile type which is orange and appears in the top of a box the \emph{top orange} type, and that in the bottom of a box the \emph{bottom orange} type. For shorthand, we will refer to macrotiles representing orange tiles simply as top or bottom orange macrotiles, and macrotiles in POC locations as POC macrotiles.
    
    %\item For a given epoch $l$, iteration $m$ in $l$, and subiteration $n$ in $m$, we refer to the box which grows for that subiteration as $\texttt{box}(l,m,n)$. Additionally, assuming the ordered enumeration of boxes in their respective epochs, iterations, and subiterations, we also refer to $\texttt{box}(l,m,n)$ as $\texttt{box}_i$ if $\texttt{box}(l,m,n)$ is the $i$th box. We refer to the sequence of radii of walls in the top (bottom) half of $\texttt{box}_i$ as its \emph{top ring pattern} (\emph{bottom ring pattern}).

    \item A hard-coded ``tail'' also grows from the seed, but in the $-x$ direction. The length of the tail is $|U|+1$, and this ensures that the scale factor of $\calUT$ must be $>1$.
\end{enumerate}

% \begin{figure}
%     \centering
%     \includegraphics[width=6.5in]{images/ring-growth.png}
%     \caption{(left to right) Pattern of growth of an example box lid/bottom with rings in locations 3,10,12, and 18.}
%     \label{fig:ring-growth}
% \end{figure}

To prove Theorem~\ref{thm:DS3DaTAM-not-IU} by contradiction, assuming that $U$ is a tile set which is universal for the class of directed Spatial aTAM system, let $\calUT = (U,\sigma_\calT,\tau)$ be the system which simulates $\calT$ using $U$, and that the scale factor of the simulation is $m$ and the assembly representation function is $R$.

\begin{figure}[htb]
    \centering
    \includegraphics[width=1.0in]{images/orange-with-fuzz.png}
    \caption{Depiction of the macrotile locations used when building sets $O_T$ and $O_B$. The grey and orange represent macrotiles, and the adjacent empty squares the fuzz regions.}
    \label{fig:orange-with-fuzz}
\end{figure}

For use in the following lemmas, we now define some useful sets and the ways in which they are computed. Let $U_m$ be the set of all possible configurations of tiles from $U$ and empty space that can be contained within an $m \times m \times m$ region, i.e. the set of all possible $m$-block macrotiles over $U$ (which may or may not be producible assemblies). Let an \emph{orange region} refer to a configuration of $8$ (macro)tiles as shown in Figure~\ref{fig:orange-with-fuzz}, representing a bottom or top orange (macro)tile along with the tile placed immediately before it, plus the $6$ adjacent (macro)tile regions where fuzz could legally grow in $\calUT$.

Let $O_B, O_T \subset U_m$ be the subset of all configurations from $U_m$ which map (under $R$) to all possible bottom, respectively top, orange regions. For each $b_i \in O_B$ where $0 \le i < |O_B|$, define the set $O_{T_i}$ and initialize it to $\emptyset$. Then, for each $b_i \in O_B$ where $0 \le i < |O_B|$, for each $t_j \in O_T$ where $0 \le j < |O_T|$, we run a simulation of a modification of $\calUT$ which uses $U$ and $\tau$, but where the seed configuration consists of $t_j$ positioned exactly one macrotile region (of dimension $m$) above $b_i$, and the simulation is run forward by placing tiles only within the macrotile regions of $b_i$, $t_j$, and between them. If nondeterminism (i.e. undirectedness) is ever encountered, that simulation is stopped and the next iteration is started. However, if a macrotile which represents (under $R$) a POC tile forms between the orange macrotiles of $b_i$ and $t_j$, then $t_j$ is added to $O_{T_i}$. This series of simulations will result in the set $O_{T_i}$, for each bottom orange region $b_i \in O_B$, representing the set of top orange regions which can cooperate with $b_i$ to grow a POC macrotile. Note that the these simulations can be run and the sets computed using time and space which depend only on the size of the tile set $U$ and the scale factor $m$.\todo{Maybe tighten this up a bit and only count types when macrotiles have added all tiles possible while staying within themselves? I don't think it's necessary and only changes things by a constant factor.}

\begin{figure}
    \centering
    \begin{subfigure}{3.2in}
        \includegraphics[width=\textwidth]{images/sub-mazes.png}
        \caption{Horizontal and vertical sub mazes of size $6\times 6$. Notice the lack of right walls on the far right side of the vertical sub mazes.}
    \end{subfigure}
    \hspace{0.2in}
    \begin{subfigure}{2.8in}
        \includegraphics[width=\textwidth]{images/formed-mazes.png}
        \caption{Examples of mazes formed by combining sub mazes.}
    \end{subfigure}
    \caption{}
    \label{fig:sub-mazes}
\end{figure}

\begin{lemma} \label{lem:gotta-make-bad-guesses}
In $\calUT$ there exist two pairs of orange top and bottom regions $b_i,b_j \in O_B$ and $t_k,t_l \in O_T$ such that $t_k \in O_{B_i}$ and $t_l \in O_{B_j}$ (i.e. $b_i$ can cooperate with $t_k$ and $b_j$ can cooperate with $t_l$ to grow POC macrotiles). (Note that it may be the case that $b_i = b_j$ and/or $t_k = t_l$.) Furthermore, in $\calUT$ there exist two maze boxes, $\texttt{maze-box}_1$ and $\texttt{maze-box}_2$, such that they each have a sealed compartment which contains $b_i$ and $t_k$ aligned with each other, and $\texttt{maze-box}_1$ contains $b_j$ aligned with a non-orange macrotile, and $\texttt{maze-box}_2$ contains $t_l$ aligned with a non-orange macrotile. Finally, there also exists a maze box $\texttt{maze-box}_3$ that contains a sealed compartment where $b_j$ is aligned with $t_l$ and they grow a POC between them.
\end{lemma}

\begin{proof}
First notice that for every integer $k \ge 1$, there is a rib of our system which grows all combinations of top and bottom $k\times k$ half mazes in every possible order of construction. To prove this lemma, we fix some sufficiently large $n$ and let $M$ be the fixed number of distinct macrotile representations of POC tiles. Now we will consider several mazes of size $2(n+2) \times 2(n+2)$, which will be described in terms of $(n+2)\times (n+2)$ quadrants which we call \emph{sub mazes}. The sub mazes we will consider are similar to those illustrated in figure \ref{fig:sub-mazes}. We call the first family of sub mazes the \emph{horizontal} sub mazes. Each horizontal sub maze has a single cooperative orange tile in the top left corner panel and is entirely made up of 4-wall panels except for a horizontal row of panels which span the width of the sub maze which form a path from one end of the sub maze to the other. Similarly, \emph{vertical} sub mazes consist of a single cooperative orange tile in the top left corner panel and are made up of 4-wall panels with the exception of a column of panels which spawn the height of the sub maze. Additionally however, vertical sub mazes also have a horizontal path from the orange cooperative tile panel to the spanning column of panels and the far right panels of the sub maze do not have a right wall. Figure \ref{fig:sub-mazes} illustrates the 4 horizontal and 4 vertical sub mazes of size $(4+2)\times (4+2)$. Notice that, in general, there are $n$ different vertical and $n$ different horizontal sub mazes of size $(n+2)\times (n+2)$. Let the \emph{empty} sub maze be the maze that is made up of all 0-wall panels.

We can now form $2(n+2) \times 2(n+2)$ mazes by combining 4 sub mazes. Consider the family of mazes that are made up of 3 horizontal sub mazes and an empty sub maze with the constraint that the sub mazes be rotated so that the orange cooperative tiles are in the center. An example is shown in figure \ref{fig:sub-mazes}. These mazes will be grown from the $\bottomrib$. Notice that there are $n^3$ of these because there are 3 independent choices between the $n$ different horizontal sub mazes. Each of these $n^3$ mazes must appear in the corresponding $\bottomrib$. Furthermore, the number of POC macrotiles is $M$. Since each maze contains 3 POC tiles, there are $M^3$ ways in which the simulator might choose to represent those POC tiles. Because we can suppose that $n^3 > M^3(C+1)$, for any arbitrary fixed $C$, since we chose $n$ to be sufficiently large, by the pigeonhole principle it must be the case that there are $C$ of these distinct mazes that appear on the $\bottomrib$ which share the same macrotile representations of their 3 POC tiles. Let $B_1, \ldots, B_C$, be these bottom mazes in $\calT$. Also, it must be the case that the sequence of bottom mazes presented by the $\bottomrib$ must be periodic. Because the counter used to repeat the $\bottomrib$ is fixed-width, it must be the case that, eventually, the simulator will have to reach its pumping length and will also have to become periodic.

Now notice that we can construct mazes from 3 vertical sub mazes similarly to be grown from the $\toprib$, and that any of these vertical mazes, when forming a maze box with any of the horizontal mazes, will admit a diffusion path for each of the three POCs as illustrated in figure \ref{fig:maze-paths}.

\end{proof}

Lemma~\ref{lem:gotta-make-bad-guesses} states that for some sealed portions of $\texttt{maze-box}_1$, and $\texttt{maze-box}_2$, the top and bottom orange regions $b_i$ and $t_k$ have the ability to cooperate to grow a POC tile when they are grown independently of all other portions of the assembly. We now use the following two lemmas to show that this must cause $\calUT$ to either be undirected or to grow an invalid assembly under $R$.

\begin{figure}
    \centering
    \includegraphics[width=5in]{images/maze-path.png}
    \caption{An example of a top half and bottom half mazes composing a maze box. The colored dots represent POC tiles in the panels. The POCs are colored the same if they can cooperate. Notice that if two POCs tiles are opposite each other and there is a path through which tiles can diffuse, it must be possible for those POCs to cooperate.}
    \label{fig:maze-paths}
\end{figure}

\begin{lemma}\label{lem:porous-boxes}
After the first tile placement in $\calUT$ in which the subassembly representing the sealed portion of $\texttt{maze-box}_1$ of Lemma~\ref{lem:gotta-make-bad-guesses} which contains aligned copies of  $b_i$ and $t_k$ maps fully to $\texttt{maze-box}_1$ in $\calT$, tiles must still be able to diffuse into one or more locations of the POC macrotile.
\end{lemma}

%[TODO: here is a high-level sketch of the proof:
%We will prove Lemma~\ref{lem:porous-boxes} by noting that the orange macrotile adjacent to the POC that is able to independently place a tile into the POC macrotiles could be the first to grow and it may or may not place that tile before the other orange macrotile completes. If diffusion into the POC macrotile was not allowed, that tile may or may not get placed, making the simulator undirected.]

[TODO: update the following proof to use maze-box notation]

\begin{proof}
Lemma~\ref{lem:porous-boxes} claims that even once $\calUT$ contains a subassembly which represents $\texttt{box}(n,i)$, even though $\texttt{box}(n,i)$ is a sealed box in $\calT$, in $\calUT$ there must still be at least one path through which tiles can diffuse into it and attach to frontier locations. To prove this, we first note that the bottom and top orange macrotiles within $\texttt{box}(n,i)$ in $\calUT$ are $b_i \in O_B$ and $t_j \in O_T$ such that $t_j \in O_{T_i}$ (by Lemma~\ref{lem:gotta-make-bad-guesses}), and that, when they are placed without any other assemblies and with one macrotile of space between them, $b_i$ and $t_j$ are capable of growing a POC macrotile between them (by definition of $O_{T_i}$). Since that is the case, at least one of them must be able to grow one or more tiles into the macrotile location between them, since empty space is not allowed to map to a tile under $R$. \todo{MJP: think through fuzz cases a bit more}
%, and just $b_i$ and $b_j$ are capable of growing a representation of a POC tile between them.
Without loss of generality, we will assume this is $b_i$ (if it was otherwise, the following argument could be trivially reflected). Furthermore, since there is an assembly sequence in $\calT$ where the bottom orange macrotile of $\texttt{box}(n,i)$ attaches before any tiles of the box lid, $\calUT$ must also be able to grow the box bottom up through $b_i$ first. (Note that since $\calUT$ must be directed, it will grow the same $b_i$ regardless of whether or not the bottom or top grows first.) However, we now consider two slightly divergent assembly sequences in $\calUT$, $\vec{\alpha_1}$ and $\vec{\alpha_2}$.

In $\vec{\alpha_1}$, after the first tile placement in which $b_i$ represents the bottom orange tile in $\calT$, no more tiles attach anywhere within the box bottom until after the box top grows to the point where $t_j$ represents the top orange tile. Note that this must be a valid assembly sequence because $\calUT$ is directed, and since $\calT$ has an assembly sequence in which the top grows completely before any portion of the bottom grows (and vice versa), the pieces of each can grow in any order and $\calUT$ must be able to model that, again remaining directed.

In contrast, in $\vec{\alpha_2}$, after the first tile placement in which $b_i$ represents the bottom orange tile in $\calT$, tiles attach within $b_i$ until the first tile can and does attach above it, in the macrotile location where a POC tile would form between $b_i$ and $t_j$. This also must be a valid assembly sequence since whichever tiles could attach in the simulation in which $O_{T_i}$ was determined must also be able to attach now because up until one or more tiles have attached within the POC macrotile, they rely only upon the tiles of $b_i$ and the fact that a path for diffusion exists, which it must because the box top has not yet grown.
Then, in $\vec{\alpha_2}$ growth continues until $t_j$ represents the top orange tile.

Now, we see that there are two valid assembly sequences in $\calUT$ in which the sealed box $\texttt{box}(m,n)$ is represented, but one of them, $\vec{\alpha_2}$, has at least one more tile in the space inside of the box which maps to a constrained subspace. Therefore, if tiles are not still able to diffuse into the locations of the POC macrotile, then $\calUT$ would not be directed, which is a contradiction to the assumption that $\calUT$ is a directed simulator of $\calT$. Therefore, Lemma~\ref{lem:porous-boxes} must be true.
\end{proof}

(Note that lemmas analogous to Lemma~\ref{lem:porous-boxes} but with $\texttt{maze-box}_1$ and $\texttt{maze-box}_2$ substituted for $\texttt{maze-box}_3$ follow immediately from Lemma~\ref{lem:gotta-make-bad-guesses} and the proof of Lemma~\ref{lem:porous-boxes}.)

\begin{lemma}\label{lem:leak-plug}
Either one or both of $b_j$ and $t_l$ have a pathway allowing tiles to diffuse through them.
\end{lemma}

\begin{proof}
[TODO: prove it...]
\end{proof}

\begin{lemma}\label{lem:unwanted-POC-growth}
A POC macrotile must be able to grow within the space representing the sealed box containing $b_i$ and $t_k$ in either $\texttt{maze-box}_1$ or $\texttt{maze-box}_2$.
\end{lemma}

\begin{proof}
To prove Lemma~\ref{lem:unwanted-POC-growth}, we show how growth can occur in $\texttt{box}(n,i)$ of the previous Lemmas which results in the POC macrotile region resolving to a POC macrotile. To do so, we simply continue assembly of assembly sequence $\vec{\alpha_2}$ used in the proof of Lemma~\ref{lem:porous-boxes}. By the definitions of $b_i$, $t_j$, and $O_{T_i}$, we know that there is a valid assembly sequence which attaches tiles only to those of macrotiles $b_i$, $t_j$, or the region of the POC macrotile between them which is capable of producing a POC macrotile which maps to a POC tile under $R$. By Lemma~\ref{lem:porous-boxes}, we know that there is a ...

SHIT!!! Growth could be allowed via holes through the orange macrotiles on both sides until cooperation occurs in the middle. The cooperation could seal the box and the representation function might only resolve the POC macrotile if and when tiles attach to the cooperating tiles on the surfaces facing the inside of the box.


%note that the POC macrotile growth would have to wait until a hole is detected in the box. However, there is no way to distinguish between a hole that will remain permanently and one which will be filled later, while also remaining directed.

%whatever could have grown into the POC macrotile to cause it to resolve to a tile must be stopped by the presence of walls from the opposite side. However, if that growth could have occurred without those walls, it could also be done before they arrive. Any mechanism which could try to detect of something must require undirectedness. [TODO: this needs to be much more clearly expressed...] Or, the POC macrotile could wait to grow until a hole is detected
\end{proof}

By Lemma~\ref{lem:unwanted-POC-growth}, $\calUT$ must be able to grow an assembly that represents an assembly that is not in $\prodasm{\calT}$, and therefore $\calUT$ does not simulate $\calT$, and thus Theorem~\ref{thm:DS3DaTAM-not-IU} is proven.
\end{proof}


==> aTAM-cant-sim-DPaTAM.tex <==
\section{The aTAM Cannot Simulate the Directed PaTAM}

\begin{theorem}\label{thm:atam-cant-sim-dpatam}
There exists a directed Planar aTAM system which cannot be simulated by any aTAM system.
\end{theorem}

\begin{proof}
We prove Theorem~\ref{thm:atam-cant-sim-dpatam} by describing a directed Planar aTAM system $\calP$ and then, by contradiction, showing that no aTAM system can simulate $\calP$.

Let $\calP = (T_\calP,\sigma_\calP,\tau)$ be the directed Planar aTAM system described as follows. At a high-level, $\calP$ grows in a series of $\stage$s. Each $\stage$ begins growth from a rectangular assembly, with the first such rectangular assembly being the seed $\sigma$. Therefore, we will refer to each of these as the ``$\seed$'' of the $\stage$. Each $\stage$ consists of the sequential growth of the segments of a $\path$, each of which is called a $\ps$. Each $\ps$ is a long, narrow rectangle which either (1) grows to some computed distance (whose computation will be discussed later) and terminates, or (2) grows until the point at which it collides with some previously grown portion of the $\path$ or the $\stage$'s $\seed$. In case (1), a new $\ps$ begins growth from the end of the previous by turning either left (L) or right (R) relative to the growth direction of the newly-terminated $\ps$. The direction, L or R, depends on the result of a computation (also to be discussed later). In case (2), by the Jordan Curve Theorem [ref?], the collision of the $\ps$ into previously placed tiles necessarily creates an ``interior'' region and an ``exterior'' region, with one being to the L, and the other to the R, relative to the growth direction of the newly-terminated $\ps$. Because $\calP$ is a system in the Planar aTAM, it is impossible for tiles to diffuse into the interior region, and thus growth within it ceases. In the exterior region, a new $\ps$ is initiated a short distance (to be discussed) backward along the direction of growth of the newly-terminated $\ps$ and perpendicular to its direction of growth.
\todo{Add a simple picture of a stage with names for the various pieces. Maybe a series of images showing cases (1) and (2).}

Throughout the growth of a $\stage$, a number $c \in \mathbb{N}$, referred to as the $\scount$ for the $\stage$, is decremented after the growth of each $\ps$ and then passed to the next $\ps$. This occurs whether or not a $\ps$ completes growth or encounters a collision. Once $c$ is decremented to $0$ (or a special case related to path collisions, to be discussed later, occurs) no more $\ps$s grow for the current stage. Instead, a process of ``filling growth'' occurs in which the concavities of the exterior region of the $\path$ are filled with tiles until a bounding rectangle is formed. At this point, the rectangle becomes the $\seed$ for the growth of the next $\stage$. This process continues infinitely, growing an infinite number of $\stage$s.

During the growth of a stage, the distance of growth of each $\ps$s, and whether a turn is made to the L or R before growth of the next $\ps$, are determined by the computation of Turing machine (TM) which is simulated within the zig-zag growth of the $\ps$. The input to the TM is the $\scount$ value $c$. The particular TM which is simulated is one of a set of $m$ \todo{Determine what $m$ is. It may only need to be 2} TMs, which we will refer to as $M_0$, $M_1 \ldots M_{m-1}$.

\subsection{Details of a $\ps$}

\begin{enumerate}
    \item Growth on a ``grid''
    \item Input: $\scount$ value $c$ (maybe $c$ begins as the width of the previous stage?)
    \item Zig-zag growth of TM $M_i$, for $0\le i < m$, where $i=0$ for the first $\ps$
    \item Extensions are by grid distance, with a column of tiles (called a $\probe$) which grows out to test for a collision, then back 
    \item Propagation and rotation of input bits
    \item Growth of $\bumper$s
    \item Termination of one $\ps$ and beginning of next
    \item Collision handling: backup to last complete set of input bits then start next $\ps$
\end{enumerate}

\subsection{Computations within $\calP$}

\begin{enumerate}
    \item Describe a program which generates a $\path$
    \item Distance
    \item Direction (L or R)
    \item Bumper type
    \item How to change computation based on bumper type after collision
\end{enumerate}

 \subsection{Completion of a $\stage$ and beginning of next}
 
 \begin{enumerate}
     \item Completion due to $\counter = 0$
     \item Completion due to insufficient space (final $\ps$ doesn't have space to rotate all bits)
     \item Filling protocol
     \item Growth of $\seed$ bumpers
     \item Initiation of next $\stage$ from a subset of the bottom side
 \end{enumerate}
 
 \subsection{Impossibility of simulation of $\calP$}
 
 We prove that no aTAM system can simulate $\calP$ by contradiction. Therefore, assume that there exists aTAM system $\calS = (T_\calS,\sigma_\calS,\tau)$ which simulates $\calP$. 
 
 We don't yet have the tools to prove the following lemma. Here are some things to think about though:
 \begin{enumerate}
     \item After some constant number of collisions with the same bumper, it must provide the same information (since it is a pumped sequence and fuzz, which may grow after each collision, is bounded)
     
     \item How to show that the same suffix, with exact same cut multiple times, must be colliding with the same pattern location...
 \end{enumerate}
\begin{lemma}
In $\calS$, there exist $\stage$s $i$ and $j$, for $i,j \in \mathbb{Z}^+$ and $j \neq j$, such that in both of them identical $\probe$s collide with the same location within a $\bumper$ pattern\todo{Define what is meant by $\bumper$ pattern}, but in $\stage$ $i$ the exterior is to the left of the collision and in $\stage$ $j$ the exterior is to the right.
\end{lemma}

Some math related to $\ps$s:
\begin{enumerate}
    \item Let $\mathcal{L} = \{L_0,L_1,L_2,\ldots L_{m-1}\}$ be a set of $m$ decidable languages over $\Sigma = \{0,1\}$, and $\mathcal{M} = \{M_0,M_1,M_2,\ldots M_{m-1}\}$ be a set of $m$ Turing machines (TMs) such that, for $0\le i < m$, TM $M_i$ decides language $L_i$.
    
    \item Furthermore, for each $L_i$, let $L_i$ be decidable in almost everywhere worst-case space complexity $n$, and $M_i$ decides $L_i$ in space $n$ almost everywhere which means that $M_i$ requires no more than $2^n$ time steps almost everywhere.
    
    \item Let $T: \mathcal{M} \times \mathbb{N} \rightarrow \mathbb{N}$ be a function which takes as input some TM $M_i$ and an input value $n$, and returns the number of steps in the computation $M_i(n)$.
    
    \item Let $O: \mathcal{M} \times \mathbb{N} \rightarrow \{0,1\}$ be a function which takes as input some TM $M_i$ and an input value $n$, and returns the output of the computation $M_i(n)$.
    
    \item Each $\path$ begins with an input $i \in \mathbb{N}$ to its first $\ps$. Such a path has the potential to grow to a length of $i$ $\ps$s, where each $\ps$ receives as input a value one less than the $\ps$ before it. We use the notation $p[j]$ to refer to the $\ps$ in $p$ whose input is $j$ for $0\le j <i$. We use $p[j:k]$, for $0\le j < k <i$, to refer to the sub-$\path$ consisting of concatenation of $p[j], p[j-1], \ldots, p[k]$.
    
    \item Each $\ps$ receives as input a total of two numbers, $i,j\in \mathbb{N}$ and performs the computation $M_i(j)$, i.e. the computation of the $i$th TM on input $j$. The value $0 \le i < m$, which is the number of TMs is a constant, and $n$ grows without bound the $stage$ number increases toward infinity. The tiles at the base of a $\ps$ encode exactly $\texttt{bin}(i)\# \texttt{bin}(j)$, which is the binary representation of $i$, followed by a delimiter, followed by the binary representation of $j$. Thus, the width of the base of a $\ps$ is $O(\log i)$.
    
    \item Each $\ps$ can:
    \begin{enumerate}
        \item grow to completion and turn L or R, depending on the result of $M_i(j)$\label{case:completion}
        \item crash into a bumper at a location causing it to switch to one of $m$ TMs for the next $\ps$ computation and turn L or R, depending on which is toward the exterior of the $\path$\label{case:crash}
        \item crash into a bumper, but not have enough space to initiate the next $\ps$, thus initiating the termination of the current $\stage$'s growth\label{case:abort}
    \end{enumerate}
    
    \item We define function $D$ such that, on input $\ps$ $p[i]$, $D(p[i])$ is L if $p[i]$ turns left, and R if $p[i]$ turns right (either due to case \ref{case:completion} or \ref{case:crash} above. If $\p[i]$ causes the $\stage$ to abort (case \ref{case:abort}) then $D(p[i])$ is undefined. We define $D^*$ as the function which takes as input a sub-$\path$ $p[i:j]$, i.e. $D^*(p[i:j])$, and returns $\{L,R\}^{i-j}$, which is the $(i-j)$-length sequence over $\{L,R\}$ representing the turns of $\p[k]$ for $i\le k < j$ in order. We call this the LR-sequence of $p[i:j]$. Note that if some $p[k]$ in $p[i:j]$ causes the stage to abort, then $D^*(p[i:j])$ is undefined.

    \item Let $p[i:j]$ be a sub-$path$ which does not abort, so $D^*(p[i:j])$ is defined. Thus the LR-sequence for $p[i:j]$ consists of $i-j$ turns. Note than an arbitrary subset of them may be due to collisions, while the rest are based on the outputs of the computations within their $\ps$s.
    
    \item As the $\stage$ number $s$ grows to infinity, there will potentially be longer and longer sub-$\path$s before $p[i:j]$, that is $p[s:i]$ will become arbitrarily long. This is true if there is an infinite sequence $S \subseteq \mathbb{N}$ such that, for each $s \in S$, $p[s:i]$ does not abort.
    
    \item Given non-aborting sub-$\path$s $p[s:i]$ and $p[i:j]$, for any $s \le k < i$ and $i \le l < j$, it may be possible for $p[l]$ to collide with $p[k]$.
    
    \item Each collision of such a $p[l]$ with a $p[k]$ has the potential to change the turn following $p[i]$ from L to R. (See Figure~\ref{fig:path-suffix-example} for an example.) If $|S| > 2^{i-j}$, it is possible for the $\ps$ $p[s:i]$ which follow each $s \in S$ to have $2^{i-j}$ unique LR-sequences.
    
    \item The width of each $\ps$ $p[i]$ is $O(\log i)$. Therefore, by the PHP, $O(2^{i-j}/\log i)$ of the $\ps$s representing $p[i]$ must have the same cut of tiles, while it is also possible for all of them to have different LR sequences.
    
    %\item Given a $\ps$ $p$ encoding number $n$, if no collisions happen or they occur only with $\ps$s grown after $p$, there will be a total of $n$ $\ps$s which grow from it with a single growth option that has no dependence on the rest of the assembly other than the $O(\log n)$ window across the base of $\ps$ $p$.
    %\item On the other extreme, if $p$ collides with a $\ps$ from its prefix, and all other $\ps$s have collisions, there are up to $m^n$ different LR-patterns for suffixes. (An LR-pattern is the sequence of L or R turns the result due to collisions.) 
\end{enumerate}



\begin{figure}
    \centering
    \begin{subfigure}{1.0in}
        \includegraphics[width=1.0in]{images/suffix-example1.png}
        %\caption{Horizontal and vertical sub mazes of size $6\times 6$. Notice the lack of right walls on the far right side of the vertical sub mazes.}
    \end{subfigure}
    \begin{subfigure}{1.5in}
       \includegraphics[width=1.5in]{images/suffix-example2.png}
        %\caption{Examples of mazes formed by combining sub mazes.}
    \end{subfigure}
    \begin{subfigure}{2.0in}
        \includegraphics[width=2.0in]{images/suffix-example3.png}
    \end{subfigure}
    \caption{An example of 3 consecutively longer $\path$s, where the sub-$\path$ $p[i:j]$ (red lines) has a different LR-sequence in each due to collisions. (a) The entire path is $p[i:j]$, and its LR-sequence is LRR, (b) there is a prefex $p[s:i]$ before $p[i:j]$, and the LR-sequence of $p[i:j]$ is now LLR, (c) the prefix is longer and the LR-sequence of $p[i:j]$ is now LLL.}
    \label{fig:path-suffix-example}
\end{figure}

Playing around with some thoughts for lemmas...

\begin{lemma}[Identical colliders lemma]\label{lem:colliders}
In $\calS$, there exist 2 distinct $\stage$s, $s_1$ and $s_2$, such that in the growth of the $\path$s simulated during those $\stage$s, $p_1$ and $p_2$, respectively, each has a subassembly representing a $\ps$ whose input was some $i \in \mathbb{N}$, which we'll refer to as $p_1[i]$ and $p_2[i]$ such that (1) $p_1[i]$ and $p_2[i]$ both terminate in collisions, (2) before the first tile is placed for the collision of either, they have identical Window Movie Lemmas for a cut across their bases, and (3) following the collision of $p_1[i]$ the path $p_1$ must turn left, and following the collison of $p_2[i]$ the path $p_2$ must turn right.
\end{lemma}

\begin{lemma}[Identical bumpers lemma]\label{lem:bumpers}
There exist a pair of $\ps$s in $\calS$, $p_1[i]$ and $p_2[i]$, which meet the conditions of Lemma\ref{lem:colliders}, and furthermore, the $\ps$s with which they collide, $p_1[j]$ and $p_2[k]$, respectively, have identical bumper patterns (todo: define a bumper pattern) and the first tiles placed from $p_1[i]$ and $p_2[j]$ which are adjacent to $p_1[j]$ and $p_2[k]$, are adjacent to tiles of the same type in the same position of the bumper patterns.
\end{lemma}

\begin{lemma}
Growth of the first macrotile after the collisions in $\stage$s $i$ and $j$ requires additional, subsequent growth outside of that macrotile.
\end{lemma}

NOTE: Growth around the exterior can only happen a constant number of times per stage since it must happen within fuzz.


TODO: must show that growth must extend arbitrarily far, which may require(?) completely identical macrotiles for the path...

Note: Interior is sealed, even in the simulator. Only a constant number of paths could go around the exterior before breaking fuzz. 

yadda yadda yadda...\footnote{We 'yadda yadded' over the best part}
\end{proof}


\begin{corollary}\label{cor:dir-atam-cant-sim-dpatam}
There exists a directed Planar aTAM system which cannot be simulated by any directed aTAM system.
\end{corollary}

Corollary~\ref{cor:dir-atam-cant-sim-dpatam} follows directly from Theorem~\ref{thm:atam-cant-sim-dpatam} since that theorem showed that no aTAM system can simulate a particular directed Planar aTAM system, and that includes all directed aTAM system.

\subsection{Thoughts for pixel-based paths}

Claims:
\begin{enumerate}
    %\item For any $l \in \mathbb{N}$, there exists a $\stage$ $s$ such that the path in $\stage$ $s$, $p_s$, grows to a length (i.e. number of $\pixel$s) which is greater than $l$, that is, $|p_s| > l$. TODO: prove this by showing that every $\stage$ can avoid aborting, or (if that's not true) that necessary sequences exist.
    
    \item $\stage$ $s$ can grow its complete $\path$, $p_s$, without aborting. TODO: prove this... if it's true

    \item If $\stage$ $s$ has pixel-scale $w$, then $|p_s| = 2^w$.
    
    \item For $0 < i < 2^w$, whether or not $\ps$ $p[i]$ collides with another $\pixel$ depends upon the $\pixel$s before it in the path, whose number is $2^w - i$. We refer to that $\path$ prefix as $p[s:i]$.
    
    \item Depending upon the values of $s$ and $i$, $|p[s:i]| >> w$, which is the width of the input to $p[i]$.
    
    \item  For a sub-$\path$ $p[i:j]$, we'll denote its collision-LR-sequence, the sequence of collisions and resulting LR turns (which are dictated by planarity), as $LRS(p[i:j])$.

    \item $|LRS(p[i:j])| \le |p[i:j]|$, can be such that $|LRS(p[i:j])| >> w$.
    
    \item The pixel-scale prevents the full collision-LR-sequence from being passed between any pair of pixels, or into the first pixel from the previous stage.
    
    \item $p[i]$ cannot know if it will collide or which direction it would need to turn if it did ... because it would have to know the positions of all previous pixels. We can show this with examples, but how to prove???
    
    \item Must show that we cannot ``pick up'' a bit of the sequence at each crash. Let $p[j]$ be the pixel into which $p[i]$ crashes. It must be that $i < j < 2^w$ (i.e. it comes before  [TODO: maybe just count upward through the $\ps$s since the scale stays the same?) $p[j]$ can't receive the necessary info that it presents for the collision...
\end{enumerate}

\subsection{Thoughts for a direction based on the computational complexity of polygon inclusion}

Perhaps we could prove that knowing whether to turn left or right after a collision requires a computation utilizing an amount of time and space greater than the simulator has available and simply use that as a contradiction...

\begin{enumerate}
    \item Let each $\stage$ consist of paths $A$ and $B$, where path $A$ grows completely, then grows a single-tile-wide path back to the center of the $\stage$, which then initiates the growth of $B$.
    \item The $\path$s $A$ and $B$ are composed of ``pixels''
    \item The input to path $A$ is some $n$, with width $\log n$, and $n$ pixels grow with each receiving as input some $i$ where $0 \le i < n$ and computing a function (via a zig-zag TM) which requires $O(\log n)$ space
    \item The input to path $B$ is $\sqrt{n}$, with width $(\log n)/2$, and $\sqrt{n}$ pixels grow with each receiving some $j$ where $0 \le j < \sqrt{n}$ and computing a function (via a zig-zag TM) which requires $O(n)$ space
    \item TODO: figure out the scale factor of pixels, maybe adjust some of those previous numbers
    \item Argue that the No Cheating Lemma\cite{DirectedNotIU} means that path $A$ cannot compute the points of path $B$
    \item Argue that $B$ cannot know the points of $A$ because there isn't room to either get the input or the set of points
    \item Give a mathematical formulation of the computational complexity of the points $A \cup B$
    \item Argue that there exist sets $A$ and $B$ such that not knowing some fraction of the points makes it impossible to determine the polygon formed by the (last?) collision of a point in $B$ with a point in $A$
    \item Argue that, by the No Cheating Lemma and the previous lemmas(?) that it is impossible for the simulator to compute the polygon formed by the paths, and therefore impossible to solve the polygon inclusion problem to determine the exterior and whether the post-collision path should turn left or right
\end{enumerate}


==> sim-def.tex <==
\section{new definition}

% System $\calS$ models system $\calT$ if for all $\alpha, \beta \in \calA[\calT]$ and $\alpha'', \beta' \in \calA[\calS]$ there exists $\alpha' \in \calA[\calS]$ such that if $R^*(\alpha'')=\alpha$ and $R^*(\beta')=\beta$ and $\alpha \to^\calT \beta$ and $\alpha''\to^\calS \beta'$ then $R^*(\alpha')=\alpha'$ and $\alpha'\to^\calS\alpha''$

% Or in a more explicitly formal notation:
% $$\forall\alpha, \beta \in \calA[\calT], \alpha'', \beta' \in \calA[\calS],\exists\alpha' \in \calA[\calS] \big[(R^*(\alpha'')=\alpha \land R^*(\beta')=\beta \land \alpha \to^\calT \beta \land \alpha''\to^\calS \beta') \implies (R^*(\alpha')=\alpha' \land \alpha'\to^\calS\alpha'')\big]$$

% We can define a formula $\psi(\alpha, \beta, \alpha', \calA[\calS]) :=$
% $$(\alpha\to^\calT\beta)\implies \big((R^*(\alpha')=\alpha) \land (\exists\beta'\in\calA[\calS](R^*(\beta') = \beta \land \alpha'\to^\calS\beta'))\big)$$

% Because of the axiom schema of specification, we can use this formula to define a set $\Pi$ of all the $\alpha'$ that satisfy it. This set is identical to the set $\Pi$ in the old definition of models given this new definition of models. Moreover, this definition also implies that for a given $\alpha\in\calA[\calT]$ there is at least one item in $\Pi$


\noindent Old definition:

\begin{definition}
\label{def-s-models-t} We say that $\mathcal{S}$ \emph{models} $\mathcal{T}$ (under $R$), and we write $\mathcal{S} \models_R \mathcal{T}$, if for every $\alpha \in \prodasm{\mathcal{T}}$, there exists $\Pi \subset \prodasm{\mathcal{S}}$ where $\Pi \neq \emptyset$ and  $R^*(\alpha') = \alpha$ for all $\alpha' \in \Pi$, such that, for every $\beta \in \prodasm{\mathcal{T}}$ where $\alpha \rightarrow^\mathcal{T} \beta$, (1) for every $\alpha' \in \Pi$ there exists $\beta' \in \prodasm{\mathcal{S}}$ where $R^*(\beta') = \beta$ and $\alpha' \rightarrow^\mathcal{S} \beta'$, and (2) for every $\alpha'' \in \prodasm{\mathcal{S}}$ where $\alpha'' \rightarrow^\mathcal{S} \beta'$, $\beta' \in \prodasm{\mathcal{S}}$, $R^*(\alpha'') = \alpha$, and $R^*(\beta') = \beta$, there exists $\alpha' \in \Pi$ such that $\alpha' \rightarrow^\mathcal{S} \alpha''$.
\end{definition}

\noindent This is the original definition using purely logical symbols and indented to be easier to read

\begin{tabbing}
    \hskip\parindent\=\hskip\parindent\=\hskip\parindent\=\hskip\parindent\=\hskip\parindent\=\kill
    $\forall \alpha \in \calA[\calT], \exists \Pi \subset \calA[\calS]\;($ \+\\
    $(\Pi \not= \emptyset)\;\land$\\
    $\forall \beta \in\calA[\calT]\;($\+\\
    $\alpha\to^\calT\beta \implies ($\+\\
    $\forall \alpha'\in\Pi, \exists\beta'\in\calA[\calS]\;(R^*(\alpha')=\alpha\;\land\;R^*(\beta')=\beta\;\land\;\alpha'\to^\calS\beta')\;\land$\\
    $\forall \alpha'', \beta'\in\calA[\calS], \exists\alpha'\in\Pi\;($\+\\
    $(\alpha''\to^\calS\beta'\;\land\;R^*(\alpha'')=\alpha\;\land\;R^*(\beta')=\beta) \implies (\alpha'\to^\calS\alpha'')$\-\\
    $)$\-\\
    $)$\-\\
    $)$\-\\
    $)$\\
\end{tabbing}

\noindent The new definition in a more expanded form is as follows:

\begin{tabbing}
    \hskip\parindent\=\hskip\parindent\=\hskip\parindent\=\hskip\parindent\=\hskip\parindent\=\kill
    $\forall \alpha, \beta \in \calA[\calT]\;($\+\\
    $\alpha\to^\calT\beta \implies ($\+\\
    $\exists \alpha', \beta'\in\calA[\calS]\;(R^*(\alpha')=\alpha\;\land\;R^*(\beta')=\beta\;\land\;\alpha'\to^\calS\beta')\;\land$\\
    $\forall\alpha'', \beta'\in\calA[\calS], \exists\alpha'\in\calA[S]\;($\+\\
    $(R^*(\alpha'')=\alpha\;\land\;R^*(\beta')=\beta\;\land\;\alpha''\to^\calS\beta')\implies(R^*(\alpha')=\alpha\;\land\;\alpha'\to^\calS\alpha'')$\-\\
    $)$\-\\
    $)$\-\\
    $)$\\
\end{tabbing}

\noindent This can be condensed to the more compact (with fewer explicit quantifiers):

\begin{tabbing}
    \hskip\parindent\=\hskip\parindent\=\hskip\parindent\=\hskip\parindent\=\hskip\parindent\=\kill
    $\forall \alpha, \beta \in \calA[\calT], \alpha''\beta_1'\in\calA[\calS]\;($\+\\
    $\exists \alpha', \beta_2'\in\calA[\calS]\;($\+\\
    $\alpha\to^\calT\beta \implies ($\+\\
    $R^*(\alpha')=\alpha\;\land\;R^*(\beta_2')=\beta\;\land\;\alpha'\to^\calS\beta_2'\;\land$\\
    $((R^*(\alpha'')=\alpha\;\land\;R^*(\beta_1')=\beta\;\land\;\alpha''\to^\calS\beta_1')\implies(\alpha'\to^\calS\alpha''))$\-\\
    $)$\-\\
    $)$\-\\
    $)$\\
\end{tabbing}

Proof of equivalence (kinda):

\begin{proof}
    Assume the new definition, fix $\alpha\in\calA[\calT]$ and define $\psi(\alpha, \beta, \alpha', \calA[\calS]) :=$
    $$ (\alpha \to^\calT\beta) \implies ((R^*(\alpha')=\alpha)\;\land\;(\exists\beta'\in\calA[\calS]\;(R^*(\beta')=\beta\;\land\;\alpha'\to^\calS\beta')))$$
    
    By the axiom schema of specification, this formula defines a set, say $\Pi$, of all $\alpha'\in\calA[\calS]$ that satisfy it. Now fix $\beta\in\calA[\calT]$ such that $\alpha\to^\calT\beta$. Given the new definition, there exists an $\alpha'\in\calA[\calS]$ such that $R^*(\alpha')=\alpha$ and such that there exists a $\beta'\in\cal[S]$ satisfying $R^*(\beta')=\beta$ and $\alpha'\to^\calS\beta'$. This means that this $\alpha'$ is a member of $\Pi$ and therefore that $\Pi\not=\emptyset$.
    
    Now let $\alpha'\in\Pi$, by the defintion of the set $\Pi$, there exists a $\beta'\in\calA[\calS]$ such that $R^*(\alpha')=\alpha$ and $R^*(\beta')=\beta$ and $\alpha'\to^\calS\beta'$, so the first condition of the old definition is met.
    
    Let $\alpha'', \beta'\in\calA[\calS]$. By the new definition, there exists an $\alpha'\in\calA[\calS]$ which satisfies the formula defining $\Pi$, such that if $\alpha''\to^\calS\beta'$ and $R^*(\alpha'')=\alpha$ and $R^*(\beta')=\beta$ then $\alpha'\to^\calS\alpha''$. This shows that the second condition of the old definition is met
\end{proof}

==> window-movie-lemmas.tex <==
\section{Variants of the Window-Movie Lemma}



\subsection{Windows}
\label{sec:windows}

In order to prove $U$ produces invalid assemblies when simulating the aforementioned system, we develop a technique called \emph{window movies} for constructing additional producible assemblies of a tile set ($U$) and seed $\sigma$, given a some initial producible assembly.
Window movies share some similarities with the proof of Theorem 3.1 in~\cite{Aggarwal-2005}, which shows that thin rectangular assemblies can be ``pumped'' to create new producible assemblies of arbitrary length.
We strengthen the technique in~\cite{Aggarwal-2005} so that assemblies can also be ``pumped down'', generating producible assemblies \emph{smaller} than the original assembly.
Besides being useful for
Theorem~\ref{thm:not-iu}, this lemma gives a general method to combine assemblies together which might be useful elsewhere.

\begin{definition}
A window $w$ is a set of edges forming a cut-set in the infinite grid graph.
\end{definition}

Given a window $w$ and an assembly $\alpha$, a window that {\em intersects} $\alpha$ is a partioning of $\alpha$ into two  configurations (i.e.\ after being split into two parts, each part may or may not be  disconnected).
In this case we say that the window $w$ cuts the assembly $\alpha$ into two configurations $\alpha_L$ and~$\alpha_R$, where $\alpha = \alpha_L \cup \alpha_R$.
Given a window $w$, its translation by a vector $\vec{c}$,  written $ w + \vec{c}$ is simply the translation of each of $w$'s elements (edges) by~$\vec{c}$.
Examples of windows are shown in Figure~\ref{fig:window}.

\begin{figure}[ht]
\centering
\includegraphics[scale=1.0]{./images/window.pdf}
\caption{Three examples of windows, shown as thick segments.
Each window partitions an assembly into two (not necessarily connected) configurations.}
\label{fig:window}
\end{figure}

For a window $w$ and an assembly sequence $\vec{\alpha}$, we define a window movie~$M$ to be the order of placement, position and glue type for each glue that appears along the window $w$ in an assembly sequence $\vec{\alpha}$.
% We extend the idea of a window to include the ordered sequence in which glues incident to the window appear during assembly, and we call this sequence a \emph{window movie}.

\begin{definition}
Given an assembly sequence $\vec{\alpha}$ and a window $w$, the associated {\em window movie} is the maximal sequence $M_{\vec{\alpha},w} = (v_{0}, g_{0}) , (v_{1}, g_{1}), (v_{2}, g_{2}), \ldots$ of pairs of grid graph vertices $v_i$ and glues $g_i$, given by the order of the appearance of the glues along window $w$ in the assembly sequence $\vec{\alpha}$.
Furthermore, if $k$ glues appear along $w$ at the same instant (this happens upon placement of a tile which has multiple  sides  touching $w$) then these $k$ glues appear contiguously and are listed in lexicographical order of the unit vectors describing their orientation in $M_{\vec{\alpha},w}$.
\end{definition}

An example of a window movie is shown in Figure~\ref{fig:window_movie1}.

\begin{figure}[ht]
\centering
\includegraphics[scale=1.0]{./images/window_movie1.pdf}
\caption{Top: A window (thick line) and an assembly sequence along the window.
Bottom: The unique induced window movie.}
\label{fig:window_movie1}
\end{figure}

%Given a window movie $M_{S,w} = (v_{0}, g_{0}) , (v_{1}, g_{1}), (v_{2}, g_{2}), \ldots$, the translation of $M_{S,w}$ by a vector $\vec{c}$, written $ M_{S,w} + \vec{c}$ is simply the translation of each of its vertices by $\vec{c}$, that is $M_{S,w} + \vec{c}= (v_{0} + \vec{c}, g_{0}) , (v_{1} + \vec{c}, g_{1}), (v_{2} + \vec{c}, g_{2}),  \ldots $.

\vspace{1ex}
\begin{lemma}[Window movie lemma]
\label{lem:windowmovie}
Let $\vec{\alpha} = (\alpha_i \mid 0 \leq i < l)$ and $\vec{\beta} = (\beta_i \mid 0 \leq i < m)$, with
$l,m\in\Z^+ \cup \{\infty\}$,
be assembly sequences in $\mathcal{T}$ with results $\alpha$ and $\beta$, respectively.
%Let $\alpha$ and $\beta$ be assemblies producible by a TAS $\mathcal{T} = (T, \sigma, \tau)$ via assembly sequences $A$ and $B$ respectively.
Let $w$ be a window that partitions~$\alpha$ into two configurations~$\alpha_L$ and $\alpha_R$, and $w' = w + \vec{c}$ be a translation of $w$ that partitions~$\beta$ into two configurations $\beta_L$ and $\beta_R$.
Furthermore, define $M_{\vec{\alpha},w}$, $M_{\vec{\beta},w'}$ to be the respective window movies for $\vec{\alpha},w$ and $\vec{\beta},w'$, and define $\alpha_L$, $\beta_L$ to be the subconfigurations of $\alpha$ and $\beta$ containing the seed tiles of $\alpha$ and $\beta$, respectively.
Then if $M_{\vec{\alpha},w} = M_{\vec{\beta},w'}$, it is the case that  the following two assemblies are also producible:
(1) the assembly $\alpha_L \beta'_R = \alpha_L \cup \beta'_R$ and
(2) the assembly $\beta'_L \alpha_R = \beta'_L \cup \alpha_R$, where $\beta'_L=\beta_L-\vec{c}$ and $\beta'_R=\beta_R-\vec{c}$.
\end{lemma}

Before proceeding, we first define some notation that will be useful for this section of the paper.

For an assembly sequence $\vec{\alpha} = (\alpha_i \mid 0 \leq i < l)$, we write $\left| \vec{\alpha} \right| = l$ (note that if $\vec{\alpha}$ is infinite, then $l = \infty$). We write $\vec{\alpha}[i]$ to denote $\vec{x} \mapsto t$, where $\vec{x}$ and~$t$ are such that $\alpha_{i+1} = \alpha_i + \left(\vec{x} \mapsto t\right)$, i.e., $\vec{\alpha}[i]$ is the placement  of tile type $t$ at position~$\vec{x}$, assuming that $\vec{x} \in \partial_{t}\alpha_i$. We define $\vec{\alpha} = \vec{\alpha} + \left(\vec{x} \mapsto t\right) = (\alpha_i \mid 0 \leq i < k + 1)$, where $\alpha_{k} = \alpha_{k-1} + \left(\vec{x} \mapsto t\right)$ if $\vec{x} \in \partial_{t}^{\tau}\alpha_i$ and undefined otherwise, assuming $\left| \vec{\alpha} \right| > 0$. Otherwise, if $\left| \vec{\alpha} \right| = 0$, then $\vec{\alpha} = \vec{\alpha} + \left(\vec{x} \mapsto t \right) = (\alpha_0)$, where $\alpha_0$ is the assembly such that $\alpha_0\left(\vec{x}\right) = t$ and is undefined at all other positions. This is our notation for appending steps to the assembly sequence $\vec{\alpha}$: to do so, we must specify a tile type $t$ to be placed at a given location $\vec{x} \in \partial_t\alpha_{i-1}$. If $\alpha_{i+1} = \alpha_i + \left(\vec{x} \mapsto t\right)$, then we write $Pos\left(\vec{\alpha}[i]\right) = \vec{x}$ and $Tile\left(\vec{\alpha}[i]\right) = t$. For a movie window $M = (v_0,g_0), (v_1,g_1), \ldots$, we write $M[k]$ to be the pair $\left(v_{k-1},g_{k-1}\right)$ in the enumeration of $M$ and $Pos\left(M[k]\right) = v_{k-1}$, where $v_{k-1}$ is a vertex of a grid graph.

\begin{proof}
We give a constructive proof by giving an algorithm for constructing an assembly sequence yielding $\alpha_L \beta_R'$. Let $\vec{\alpha}$ and $\vec{\beta}$ be the assembly sequences of $\alpha$ and $\beta$, respectively.
Intuitively, the algorithm performs a lossy merge of $\vec{\alpha}$ and $\vec{\beta}$, ignoring assembly sequence steps of $\vec{\alpha}$ (respectively, $\vec{\beta}$) that place tiles in $\alpha_R$ ($\beta_L'$).
Without loss of generality, and for notational simplicity,  let~$w$ be a window such that $M_{\vec{\alpha},w} = M_{\vec{\beta},w}$. In other words,  the common window movie of $\vec{\alpha}$ and $\vec{\beta}$ occur at the same location in the plane, and thus since $\vec{c} = \vec{0}$, $\beta_L = \beta_L'$ and $\beta_R = \beta_R'$. % hopefully this addresses translation cleanly. One can generalize by translating seed of $\beta$ appropriately.
Let~$M$ be the sequence of steps in the window movie $M_{\vec{\alpha},w}$.
The algorithm in Figure \ref{fig:algo-seq} describes how to produce a new valid assembly sequence $\vec{\gamma}$.

%% \begin{verbatim} **)
%% Initialize i, j, k = 0 **)
%% Initialize sequence S = A[0] **)
%% While k < M.length: **)
%%     If M[k] involves a tile in \alpha_L/\beta_L: **)
%%         While i < A.length and A[i] != M[k]: **)
%%             if A[i] places a tile in \alpha_L: **)
%%                 Append A[i] to S **)
%%             ++i **)
%%         Add A[i] to S **)
%%     Else: **)
%%         While j < B.length and B[j] != M[k]: **)
%%             if B[j] places a tile in \beta_R: **)
%%                 Append B[j] to S **)
%%             ++j **)
%%         Add B[j] to S **)
%%     ++k **)
%% return S **)
%% \end{verbatim} **)
\begin{figure}[t]
\begin{algorithm}[H]
\SetAlgoLined
Initialize $i$, $j$, $k = 0$ and $\vec{\gamma}$ to be empty

\While{$i<|\vec{\alpha}|$  { \bf or }  $j<|\vec{\beta}|$}{  %k $<$ M.length
  \If{$Pos(M[k]) \in \dom{\alpha_L}$}{ %/$\beta_L$
    \While{$i < |\vec{\alpha}|$ and $Pos(\vec{\alpha}[i])\neq Pos(M[k])$}{
      \If{$Pos(\vec{\alpha}[i]) \in \dom{\alpha_L}$}{$\vec{\gamma} = \vec{\gamma} + \vec{\alpha}[i]$}
      $i = i + 1$
    }
    \If{$i<|\vec{\alpha}|$}{
      $\vec{\gamma} = \vec{\gamma} + \vec{\alpha}[i]$

      $i = i + 1$
    }
  }
  \ElseIf{$Pos(M[k]) \in \dom{\beta_R}$}{
    \While{$j<|\vec{\beta}|$ and $Pos(\vec{\beta}[j])\neq Pos(M[k])$}{
      \If{$Pos(\vec{\beta}[j]) \in \dom{\beta_R}$}{
        $\vec{\gamma} = \vec{\gamma} + \vec{\beta}[j]$}

        $j = j + 1$

    }
    \If{$j<|\vec{\beta}|$}{
      $\vec{\gamma} = \vec{\gamma} + \vec{\beta}[j]$

      $j = j + 1$
    }
  }
  \ElseIf{$k\geq |M|$}{
    \If{$i<|\vec{\alpha}|$}{
      $\vec{\gamma} = \vec{\gamma} + \vec{\alpha}[i]$

      $i = i + 1$
    }
    \If{$j<|\vec{\beta}|$}{
      $\vec{\gamma} = \vec{\gamma} + \vec{\beta}[j]$

      $j = j + 1$
    }
  }

  $k = k + 1$
}
\Return $\vec{\gamma}$

\end{algorithm}
\caption{The algorithm to produce a valid assembly sequence $\vec{\gamma}$.}
\label{fig:algo-seq}
\end{figure}

If we assume that  the assembly sequence  $\vec{\gamma}$ ultimately produced by the algorithm is valid, then the result of $\vec{\gamma}$  is indeed  $\alpha_L \beta_R$, since for every tile in~$\alpha_L$ and $\beta_R$, the algorithm adds a step to the sequence $\vec{\gamma}$ involving the addition of this tile to the assembly. However, we need to prove that  the assembly sequence $\vec{\gamma}$  is valid,  it may be the case that either: 1. there is insufficient bond strength between the tile to be placed and the existing neighboring tiles, or 2. a tile is already present at this location.
Case 2 is a non-issue, as locations in $\alpha_L$ and $\beta_L$ only have tiles from $\alpha_L$ placed in them, and locations in $\alpha_R$ and $\beta_R$ only have tiles from $\beta_R$ placed in them.
Case 1 is more difficult, and is where the remainder of the proof is spent.

Formally, we claim the following: at each step of the algorithm, the current version of $\vec{\gamma}$ at this step is a valid assembly sequence whose result is a producible subassembly of $\alpha_L \beta_R$.
Note that the outer loop of the algorithm iterates through all steps of $\vec{\alpha}$ and $\vec{\beta}$, such that at any point of adding $\vec{\alpha}[i]$ (or $\vec{\beta}[j]$) to $\vec{\gamma}$, all steps of the window movie occurring before $\vec{\alpha}[i]$ ($\vec{\beta}[j]$) in $\vec{\alpha}$ ($\vec{\beta}$) have occurred.
Similarly, all tiles in $\alpha_L$ (or $\beta_R$) added to $\alpha$ ($\beta$) before step $i$ ($j$) in the assembly sequence have occurred.

So if the $Tile\left(\vec{\alpha}[i]\right)$ that is added to the subassembly of $\alpha$ produced after $i-1$ steps, can bond at a location in $\alpha_L$ to form a $\tau$-stable assembly, the same tile added to the producible assembly of  $\vec{\gamma}$  must also bond to the same location in  $\vec{\gamma}$, as the neighboring glues consist of (i) an identical set of glues from tiles in the subassembly of $\alpha_L$ and (ii) glues on the side of the window movie containing~$\alpha_R$.  Similarly, the tiles of $\beta_R$ must also be able to bind.

So the assembly sequence of $\vec{\gamma}$ is valid, i.e.\ every addition to $\vec{\gamma}$ adds a tile to the assembly  to form a new producible assembly.
Since we have a valid assembly sequence, as argued above, the finished producible assembly is~$\alpha_L \beta_R$.
\end{proof}

In the proof, we used the two identical window movies to ensure each step in the constructed assembly sequence was valid, i.e.\ the proposed tile could attach at the specified location.
However, if a pair of incident glues in the window movie are not identical, then they are never used to ensure a proposed tile can attach.
Using this observation, we define a restricted form of  window movie, called a \emph{bond-forming submovie}, which consists  of only those steps of the window movie that place glues that eventually form positive-strength bonds in the assembly.
Every window movie $M$ has a unique bond-forming submovie ${\cal B}(M)$, and Lemma~\ref{lem:windowmovie} can be strengthened by relaxing the requirement that the window movies $M_{\vec{\alpha}, w} = M_{\vec{\beta}, w'}$ match:

\begin{corollary}
\label{cor:windowmovie}
The statement of Lemma~\ref{lem:windowmovie} holds if the window movies $M_{\vec{\alpha},w}$ and $M_{\vec{\beta},w'}$ are replaced by  their bond-forming submovies ${\cal B}\left(M_{\vec{\alpha},w}\right)$ and ${\cal B}\left(M_{\vec{\beta},w'}\right)$.
\end{corollary}

\begin{proof}
The matching window movies $M_{\vec{\alpha},w}$ and $M_{\vec{\beta},w'}$ in the proof of Lemma~\ref{lem:windowmovie} are  used  only to prove that for each step (tile addition) of $\vec{\alpha}$ or $\vec{\beta}$ that is appended to the sequence $\vec{\gamma}$, the tile can attach at the new proposed location.
For each step of $M_{\vec{\alpha},w} = M_{\vec{\beta},w'}$, either the step is in ${\cal B}\left(M_{\vec{\alpha},w}\right) = {\cal B}\left(M_{\vec{\beta}, w'}\right)$ or not.
If so, the proof is unchanged.

Otherwise, if not, the tile will not form a bond with any glue (i.e.\ tile) on the other side of the window, since the step is not in ${\cal B}\left(M_{\vec{\alpha}, w}\right)$.
Furthermore, the set of glues incident to $Pos(\vec{\alpha}[i])$ (respectively, $Pos(\vec{\beta}[j])$) and forming positive strength bonds is identical to the set when $\vec{\alpha}[i]$ ($\vec{\beta}[j]$) is added to $\vec{\gamma}$ in the proof of Lemma~\ref{lem:windowmovie}, as all elements of $\vec{\alpha}$ ($\vec{\beta}$) preceeding $\vec{\alpha}[i]$ ($\vec{\beta}[j]$) have already been added to $\vec{\gamma}$.
\end{proof}



